Dynamic Power Splitting for SWIPT with Nonlinear Energy Harvesting in Ergodic Fading Channel

We study the dynamic power splitting for simultaneous wireless information and power transfer (SWIPT) in the ergodic fading channel. Considering the nonlinearity of practical energy harvesting circuits, we adopt the realistic nonlinear energy harvesting (EH) model rather than the idealistic linear EH model. To characterize the optimal rate-energy (RE) tradeoff, we consider the problem of maximizing the R-E region, which is nonconvex. We solve this challenging problem for two different cases of the channel state information (CSI): (i) when the CSI is known only at the receiver (the CSIR case) and (ii) when the CSI is known at both the transmitter and the receiver (the CSI case). For these two cases, we develop the corresponding optimal dynamic power splitting schemes. To address the complexity issue, we also propose the suboptimal schemes with low complexities. Comparing the proposed schemes to the existing schemes, we provide various useful and interesting insights into the dynamic power splitting for the nonlinear EH. Furthermore, we extend the analysis to the scenarios of the partial CSI at the transmitter and the harvested energy maximization. Numerical results demonstrate that the proposed schemes significantly outperform the existing schemes and the proposed suboptimal scheme works very close to the optimal scheme at a much lower complexity.

==> Tex/DPS_csir_double.tex <==
\section{Dynamic Power Splitting for Nonlinear EH with CSIR}
\label{sec_P_EH}

In this section, we first derive the optimal solution to (P1).
Then we propose a suboptimal solution to (P1) with low complexity.
Finally, we compare the proposed scheme to the existing schemes.

%\begin{figure*}[t]
%\begin{align}
%\end{cases}.
%\end{align}
%\hrulefill
%\end{figure*}


\subsection{Optimal Solution to (P1)}

In order to solve the problem (P1) optimally and efficiently,
we exploit the time-sharing condition proposed in \cite{Yu}.
To this end, first, we define the time-sharing condition.
\begin{definition}[\textit{\cite[Definition 1]{Yu}}]
Let $\{ P_{x, \nu} , \rho_{ x, \nu} \} $ and $\{ P_{y, \nu} , \rho_{y, \nu} \}$ denote the optimal solutions to the problem (P2) when $ ( Q, P_{\rm avg} ) = ( Q_{x} , \overline{P}_{x} ) $ and $( Q, P_{\rm avg} ) = (Q_{y}, \overline{P}_{y} )$, respectively. It is said that (P2) satisfies the \textit{time-sharing} condition (or time-sharing property) if there exists a feasible solution $\{ P_{z, \nu} , \rho_{z, \nu} \}$
such that $\mathbb{E} [  Q_{\nu}^{\texttt{NL}} (  P_{z, \nu}, \rho_{z, \nu}   )  ] \geq \theta Q_{x} + (1 - \theta) Q_{y}$, $ \mathbb{E} [ P_{z, \nu} ] \leq  \theta \overline{P}_{x}  + (1 - \theta) \overline{P}_{y} $,
and $ \mathbb{E} [ R_{\nu} ( P_{z, \nu} , \rho_{z, \nu}) ] \geq  \theta \mathbb{E} [ R_{\nu} ( P_{x, \nu} , \rho_{x, \nu}) ] + (1 - \theta) \mathbb{E} [ R_{\nu} ( P_{y, \nu} , \rho_{y, \nu}) ] $ for any $0 \leq \theta \leq 1$.
Since the problem (P1) is a special case of (P2), it is said that (P1) satisfies the time-sharing condition if the time-sharing property holds in (P2) when $P_{\nu} = P_{\rm avg}$, $\forall \nu$.
\null \hfill $\blacksquare$
\end{definition}

%The time-sharing condition means that the optimal objective value of (P1) is a concave function of the long-term power threshold $P_{\rm avg}$, not the transmit power $\{ P_{\nu} \}$ to be optimized.
A useful fact is that if an optimization problem satisfies the time-sharing condition,
then the strong duality always holds, i.e., the duality gap is always zero, regardless of the convexity of the problem \cite[Theorem 1]{Yu}.
In the following, we establish the time-sharing property of (P1).
\begin{lemma}
\label{lem_1}
In the problem (P1), the time-sharing condition is satisfied.
\end{lemma}
\begin{IEEEproof}
See Appendix \ref{proof_lems_1_2}.
\end{IEEEproof}

%From Lemma \ref{lem_1}, the optimal solution to (P1) can be obtained by using the Lagrange duality method.
By Lemma \ref{lem_1}, it is possible to obtain the optimal solution to (P1) using the Lagrange duality method.
However, even if the Lagrange duality method can be used, it is still difficult to derive the solution to (P1) because the Lagrangian is still a nonconvex function of $\{ \rho_{\nu} \}$.
To overcome this difficulty, we take the following approach: we first classify the conditions of the channel power gain $h_{\nu}$ into the five mutually exclusive cases,
and then, we derive the optimal solution in each case.
Taking this approach, we have the following result.
\begin{theorem}
\label{thm_1}
The solution to (P1) is given by (\ref{rho_NL})
\begin{figure*}[t]
\begin{align}
\label{rho_NL}
\rho_{\nu}^{\texttt{NL}}  = \begin{cases}  0 ,   &   \rm{for~Case~1}  \\
    \begin{cases}  \rho_{{\rm o}, \nu}^{\texttt{NL}} ,  &  {\rm if} ~  R_{\nu} ( P_{\rm avg}, \rho_{{\rm o}, \nu}^{\texttt{NL}} )  + \lambda^{\texttt{NL}} Q_{\nu}^{\texttt{NL}} ( P_{\rm avg}, \rho_{{\rm o}, \nu}^{\texttt{NL}} ) >  R_{\nu} ( P_{\rm avg} , 0 )   \\ 0, & {\rm otherwise}  \end{cases},  & \rm{for~Case~2}  \\
    \begin{cases}  1 ,  &  {\rm if}  ~   \lambda^{\texttt{NL}} Q_{\nu}^{\texttt{NL}} ( P_{\rm avg} , 1 ) >  R_{\nu} ( P_{\rm avg} , 0 )  \\ 0, & {\rm otherwise}  \end{cases},  & \rm{for~Case~3} \\
    \rho_{{\rm o}, \nu}^{\texttt{NL}}   ,   &   \rm{for~Case~4}  \\
    1  ,   &   \rm{for~Case~5}
\end{cases}.
\end{align}
\hrulefill
\begin{align}
\label{rho_NL_cases}
\begin{aligned}
& \gamma ( h_{\nu} )  \geq \frac{\lambda^{\texttt{NL}}}{4}   && \quad {\rm for ~ Case ~ 1}  \\
& \lambda^{\texttt{NL}} f ( 0 ) \leq g ( h_{\nu} ) , ~   \lambda^{\texttt{NL}} f ( h_{\nu} )  <  g ( 0 ) ,  ~ {\rm and} ~  \gamma ( h_{\nu} ) < \frac{\lambda^{\texttt{NL}}}{4}  && \quad {\rm for ~ Case ~ 2} \\
& \lambda^{\texttt{NL}} f ( 0 ) \leq g ( h_{\nu} ) ~ {\rm and} ~   \lambda^{\texttt{NL}} f ( h_{\nu} )  \geq  g ( 0 )   && \quad {\rm for ~ Case ~ 3} \\
& \lambda^{\texttt{NL}} f ( 0 ) > g ( h_{\nu} ) , ~   \lambda^{\texttt{NL}} f ( h_{\nu} )  <  g ( 0 ) ,  ~ {\rm and} ~  \gamma ( h_{\nu} ) < \frac{\lambda^{\texttt{NL}}}{4}  && \quad {\rm for ~ Case ~ 4} \\
& \lambda^{\texttt{NL}} f ( 0 ) > g ( h_{\nu} ) ~ {\rm and} ~ \lambda^{\texttt{NL}} f ( h_{\nu} ) \geq  g ( 0 )  && \quad {\rm for ~ Case ~ 5}. \\
\end{aligned}
\end{align}
\hrulefill
\end{figure*}
where $\rho_{{\rm o}, \nu}^{\texttt{NL}} $ is the root of the following equation:
\begin{align}
\label{rho_opt}
& \lambda^{\texttt{NL}} \Psi_{\nu} ( P_{\rm avg}, x  ) \left(  1 - \Psi_{\nu} ( P_{\rm avg}, x  ) \right) = \frac{1 - \Omega }{  P_{s} T a \left(  (1 - x ) h_{\nu} P_{\rm avg} + \sigma^{2} \right) }
\end{align}
over $ x \in \left(  \frac{b}{h_{\nu} P_{\rm avg}} , 1 \right) $.
Also, the Cases 1--5 are given by (\ref{rho_NL_cases}) (shown at the top of the next page),
where $ f ( x ) =   \frac{ e^{ - a ( x P_{\rm avg} - b ) }  }{  \left( 1 + e^{ - a ( x P_{\rm avg} - b ) } \right)^{2} }  $, $ g ( x ) =  \frac{1 - \Omega }{ P_{s} T a ( x P_{\rm avg} + \sigma^{2} ) } $, and $ \gamma( x ) =  \frac{1 - \Omega }{ P_{s} T a \left( \max \{ x P_{\rm avg} - b , 0 \} + \sigma^{2} \right) } $.
The constant $ \lambda^{\texttt{NL}} > 0 $ is determined such that $\mathbb{E} [   Q_{\nu}^{\texttt{NL}} ( P_{\rm avg} , \rho_{\nu}^{\texttt{NL}} ) ]  = Q$.
\end{theorem}
\begin{IEEEproof}
See Appendix \ref{proof_thm_1}.
\end{IEEEproof}


From Theorem \ref{thm_1}, the optimal solution to (P1) can be efficiently computed.
Specifically, at each fading state $\nu$, one can determine the optimal power splitting ratio $ \rho_{\nu}^{\texttt{NL}} $ according to (\ref{rho_NL})
by simply checking which case the channel power gain $h_{\nu}$ falls into (through the functions $f(\cdot)$, $g(\cdot)$, and $\gamma(\cdot)$).
In the proposed solution, the positive scalars $ \lambda^{\texttt{NL}}$ and $ \{ \rho_{\nu}^{\rm opt} \} $ needs to be computed numerically
by solving the nonlinear equations of $ \mathbb{E} [   Q_{\nu}^{\texttt{NL}} ( P_{\rm avg} , \rho_{\nu}^{\texttt{NL}} ) ]  = Q $ and (\ref{rho_opt}), respectively.
Since $ \mathbb{E} [   Q_{\nu}^{\texttt{NL}} ( P_{\rm avg} , \rho_{\nu}^{\texttt{NL}} ) ]  $ is a monotonic function of $\lambda^{\texttt{NL}}$,
the value of $\lambda^{\texttt{NL}}$ can be calculated efficiently by the subgradient method 
as follows \cite{Yu}: $\lambda^{i+1}  =  \max \left\{  \lambda^{ i}  -  s^{i}  \big( \mathbb{E} [   Q_{\nu}^{\texttt{NL}} ( P_{\rm avg} , \rho_{\nu}^{\texttt{NL}} ) ]  - Q \big) , 0  \right\}$,
where $i$ denotes the iteration number, $ \lambda^{i}$ the value of $\lambda^{\texttt{NL}}$ at the $i$th iteration, and $s^{i} > 0$ the step size at the $i$th iteration.
The complexity of finding $\lambda^{\texttt{NL}}$ is given by $\mathcal{O} ( 1^{2} ) = \mathcal{O} ( 1 )$ \cite{Boyd}.
Also, the value of $ \rho_{{\rm o} , \nu}^{\texttt{NL}} $ can be found efficiently via the one-dimensional searching, e.g., the bisection method, 
of which complexity is at most $ \mathcal{O} ( K ) $ \cite{Boyd}, where the parameter $ K > 1$ is inversely proportional to the tolerance.


Overall, the computational complexity to solve (P1) is given by $\mathcal{O} (K N)$.
Note that the complexity of the proposed solution is linear in the number $N$ of fading blocks,
and thus, it is much lower than the exponential complexity $ \mathcal{O} ( M^{N} ) $ required by the exhaustive searching, where the parameter $M \geq 2$ is determined by the searching resolution.
Since $N$ is large in practice, the complexity reduction by Theorem \ref{thm_1} is indeed significant.


\subsection{Suboptimal Solution to (P1)}

The complexity of the optimal solution to (P1) in Theorem \ref{thm_1} is low.
Unfortunately, the complexity of the solution in Theorem \ref{thm_1} might not be actually very low,
because the complexity is proportional to both $N$ and $K$.
For example, when $K \geq N$, the complexity is higher than $\mathcal{O} ( N^{2})$.
In the practical fading scenario, it is very desirable to achieve the complexity in the order of $\mathcal{O} (N)$,
which is proportional only to the number $N$ of the fading blocks \cite{Yu}.
However, in (P1), it is generally challenging to reduce the complexity while guaranteeing the optimality.
To address this issue, in this subsection, we propose a suboptimal solution to (P1) in closed form (up to the Lagrange multiplier $\lambda^{\texttt{NL}}$),
which turns out to be asymptotically optimal in the low SNR region.

The fundamental idea is to maximize the lower bound of the average rate rather than the actual average rate.
To this end, in the following, we first derive a lower bound of the average rate.
\begin{lemma}
\label{lem_lb}
The objective function of the problem (P1) is lower bounded by
\begin{align}
\label{R_lb}
\mathbb{E} \left[  R_{\nu} ( P_{\rm avg} , \rho_{\nu}  )  \right]  \geq \mathbb{E} \left[  (1 - \rho_{\nu} ) R_{\nu} ( P_{\rm avg} , 0  ) \right]  .
\end{align}
\end{lemma}
\begin{IEEEproof}
Since $ R_{\nu} ( P_{\rm avg} , \rho_{\nu}  ) $ is concave in $ (1 - \rho_{\nu}) $ \cite{Zhou13}, it follows that $ R_{\nu} ( P_{\rm avg} , \rho_{\nu}  ) \geq (1 - \rho_{\nu} ) R_{\nu} ( P_{\rm avg} , 0  ) $, $\forall \nu$ \cite{Boyd}.
\end{IEEEproof}

The lower bound of (\ref{R_lb}) becomes tight when $\rho_{\nu} \in \{ 0,1 \}$, $\forall \nu$.
Replacing the objective function of (P1) by the lower bound,
we can formulate the following problem:
\begin{subequations}
\label{P1_}
\begin{align}
\label{P1_obj_}
{\rm (P1'):}  \quad  \underset{ 0 \leq \rho_{\nu} \leq 1,  \forall \nu }{\texttt{max}} & \quad \mathbb{E} \left[ (1 - \rho_{\nu} ) R_{\nu} ( P_{\rm avg} , 0  )  \right]   \\
\label{P1_const_1_}
\texttt{s.t.}  &  \quad  \mathbb{E} \left[  Q_{\nu}^{\texttt{NL}} (  P_{\rm avg} , \rho_{\nu}  )  \right] \geq Q.
\end{align}
\end{subequations}

In the following, the solution to (P1') is derived.
\begin{theorem}
\label{thm_2}
The solution to (P1') is given by (\ref{rho_NL_so}) (shown at the top of the next page),
\begin{figure*}[t]
\begin{align}
\label{rho_NL_so}
\rho_{\nu}^{\texttt{NL}'}  = \begin{cases}  0 ,   &   \rm{for~Case~1'}  \\
    \begin{cases}  \rho_{{\rm so}, \nu}^{\texttt{NL}} ,  &  {\rm if} ~ (1 - \rho_{{\rm so}, \nu}^{\texttt{NL}}) R_{\nu} ( P_{\rm avg}, 0 )  + \lambda^{\texttt{NL}} Q_{\nu}^{\texttt{NL}} ( P_{\rm avg}, \rho_{{\rm so}, \nu}^{\texttt{NL}} ) > R_{\nu} ( P_{\rm avg}, 0 )   \\ 0, & {\rm otherwise}  \end{cases},  & \rm{for~Case~2'}  \\
    \begin{cases}  1 ,  &  {\rm if}  ~ \lambda^{\texttt{NL}} Q_{\nu}^{\texttt{NL}} ( P_{\rm avg}, 1 ) > R_{\nu} ( P_{\rm avg}, 0 )  \\ 0, & {\rm otherwise}  \end{cases},  & \rm{for~Case~3'} \\
    \rho_{{\rm so}, \nu}^{\texttt{NL}}  ,   &   \rm{for~Case~4'}  \\
    1  ,   &   \rm{for~Case~5'}
\end{cases}.
\end{align}
\hrulefill
\end{figure*}
where the Cases 1'--5' are given by 
\begin{align}
\label{rho_NL_so_cases}
\begin{aligned}
& z ( h_{\nu} ) \geq  \frac{\lambda^{\texttt{NL}}}{4}    && \quad {\rm for ~ Case ~ 1'}   \\
& \max \left\{ \lambda^{\texttt{NL}} f ( h_{\nu} ), \lambda^{\texttt{NL}} f ( 0 )  \right\} < z ( h_{\nu} )  < \frac{\lambda^{\texttt{NL}}}{4}  && \quad {\rm for ~ Case ~ 2'}  \\
& \lambda^{\texttt{NL}} f ( 0 )  \leq  z ( h_{\nu} )  \leq \lambda^{\texttt{NL}} f ( h_{\nu} )  && \quad {\rm for ~ Case ~ 3'}  \\
& \lambda^{\texttt{NL}} f ( h_{\nu} )  <  z ( h_{\nu} )  < \lambda^{\texttt{NL}} f ( 0 )  && \quad {\rm for ~ Case ~ 4'}  \\
& z ( h_{\nu} )  \leq   \min \left\{ \lambda^{\texttt{NL}} f ( h_{\nu} ), \lambda^{\texttt{NL}} f ( 0 )  \right\}  && \quad {\rm for ~ Case ~ 5'}  .
\end{aligned}
\end{align}
In (\ref{rho_NL_so_cases}), $ f ( x ) =   \frac{ e^{ - a ( x P_{\rm avg} - b ) }  }{  \left( 1 + e^{ - a ( x P_{\rm avg} - b ) } \right)^{2} }  $ and $ z ( x ) =  \frac{1 - \Omega }{ P_{s} T a x P_{\rm avg} } \log_{2} \left(  1 + \frac{x P_{\rm avg}}{\sigma^{2}} \right) $.
Also, $\rho_{{\rm so}, \nu}^{\texttt{NL}}$ is given by
\begin{align}
\label{rho_subopt}
\rho_{{\rm so}, \nu}^{\texttt{NL}}  =  \frac{1}{h_{\nu} P_{\rm avg}} \left( - \frac{1}{a}  \ln \left(  \frac{ 2 }{  1 + \sqrt{ 1 - \frac{ 4 z ( h_{\nu} ) }{ \lambda^{\texttt{NL}} } }  } - 1 \right) + b \right).
\end{align}
The constant $ \lambda^{\texttt{NL}} > 0 $ is determined such that $\mathbb{E} [   Q_{\nu}^{\texttt{NL}} ( P_{\rm avg} , \rho_{\nu}^{\texttt{NL}'} ) ]  = Q$.
\end{theorem}
\begin{IEEEproof}
The result can be proved by following the similar procedures in Appendix \ref{proof_thm_1} and replacing the objective function $ \mathbb{E} \left[  R_{\nu} ( P_{\rm avg} , \rho_{\nu}  )  \right]  $ by the lower bound $\mathbb{E} \left[ (1 - \rho_{\nu} ) R_{\nu} ( P_{\rm avg} , 0  )  \right]$, where $\rho_{{\rm so}, \nu}^{\texttt{NL}}$ in (\ref{rho_subopt}) is given by the solution of the equation $ \Psi_{\nu} ( P_{\rm avg}, x  ) =  \frac{1}{2} + \sqrt{ \frac{1}{4} - \frac{z(h_{\nu})}{\lambda^{\texttt{NL}}} } $ over $ x \in \Big( \frac{b}{h_{\nu} P_{\rm avg}},  1 \Big) $.
\end{IEEEproof}

Note that the solution in Theorem \ref{thm_2} can be computed more efficiently than the optimal solution in Theorem \ref{thm_1}:
only a single positive scalar $ \lambda^{\texttt{NL}} $ needs to be computed numerically.
Specifically, the complexity of the solution in Theorem \ref{thm_2} is given by $\mathcal{O} (N)$, which is proportional only to $N$, and thus, is lower than the complexity of the optimal solution.
But, the solution in Theorem \ref{thm_2} is generally suboptimal to (P1) because the lower bound of (\ref{R_lb}) is not always tight.
Interestingly and fortunately, we can show that the solution in Theorem \ref{thm_2} is asymptotically optimal in the low SNR regime. 
\begin{lemma}
\label{lem_optimality}
When $ \frac{ P_{\rm avg} }{ \sigma^{2} } \rightarrow 0 $, the solution in Theorem \ref{thm_2} is optimal to (P1).
%i.e., $\rho_{\nu}^{\texttt{NL}'} \rightarrow \rho_{\nu}^{\texttt{NL}}$, $\forall \nu$.
\end{lemma}
\begin{IEEEproof}
It follows that $  R_{\nu} ( P_{\rm avg} , \rho_{\nu}  ) \rightarrow \frac{ (1 - \rho_{\nu}) h_{\nu} P_{\rm avg} }{ \sigma^{2} \ln 2 } $ and $ (1 - \rho_{\nu} ) R_{\nu} ( P_{\rm avg} , 0  ) \rightarrow \frac{ (1 - \rho_{\nu}) h_{\nu} P_{\rm avg} }{ \sigma^{2} \ln 2 } $ as $ \frac{ P_{\rm avg} }{ \sigma^{2} } \rightarrow 0 $ \cite{Tse}.
Thus, when $ \frac{ P_{\rm avg} }{ \sigma^{2} } \rightarrow 0 $, the gap between the actual objective value of (P1) and the lower bound of (\ref{R_lb}) approaches zero, i.e., $ R_{\nu} ( P_{\rm avg} , \rho_{\nu}  ) - (1 - \rho_{\nu} ) R_{\nu} ( P_{\rm avg} , 0  ) \rightarrow 0 $, implying that the solution in Theorem \ref{thm_2} is optimal to (P1). 
\end{IEEEproof}

Although we can mathematically show the optimality of the solution in Theorem \ref{thm_2} only in the low SNR range, 
the numerical results in Section \ref{numerical_result} will suggest that the performance of this solution is essentially the same as the optimal performance even in the moderate to high SNR range.
%this solution provides eseentially the same performance as the optimal solution in Theorem \ref{thm_1} even in the moderate to high SNR range.
%the performance of this solution is essentially the same as the optimal performance even in the moderate to high SNR range.
%this scheme actually performs very well and its performance is essentially the same as the optimal performance even in the moderate to high SNR range.


\subsection{Comparisons to Existing Schemes}
\label{sec_P_EH_comp}

In this subsection, to obtain the insights, we compare the proposed scheme to the existing schemes of \cite{Kang_2}, \cite{Liu_dps}.
For comparison, in the following, we first present the existing dynamic power splitting scheme for the linear EH \cite[Proposition 4.1]{Liu_dps}:
\begin{align}
\label{rho_L}
\rho_{\nu}^{\texttt{L}}  =  \begin{cases} \rho_{{\rm o}, \nu}^{\texttt{L}}  ,  &  {\rm if}  ~  h_{\nu}  >  x_{1}^{\texttt{L}}  \\ 0, & {\rm otherwise}  \end{cases}
\end{align}
where $ \rho_{{\rm o}, \nu}^{\texttt{L}} = 1 - \frac{1}{h_{\nu} P_{\rm avg}} \left( \frac{1}{ \zeta \lambda^{\texttt{L}} } - \sigma^{2} \right) $.
%\begin{align}
%\rho_{{\rm o}, \nu}^{\texttt{L}} = 1 - \frac{1}{h_{\nu} P_{\rm avg}} \left( \frac{1}{ \zeta \lambda^{\texttt{L}} } - \sigma^{2} \right).
%\end{align}
Also, $x_{1}^{\texttt{L}} = \frac{1}{ P_{\rm avg} }  \left( \frac{1}{ \zeta \lambda^{\texttt{L}} } - \sigma^{2} \right)$.
The constant $ 0 < \lambda^{\texttt{L}} \leq \frac{1}{\zeta \sigma^{2}} $ is determined such that $\mathbb{E} [   Q_{\nu}^{\texttt{L}} ( P_{\rm avg} , \rho_{\nu}^{\texttt{L}} ) ]  = Q$.
Next, we present the existing mode switching scheme for the nonlinear EH \cite[Lemma 2]{Kang_2}:
\begin{align}
\label{ms_NL}
\varrho_{\nu}^{\texttt{NL}}  = \begin{cases}  1 ,  & {\rm if} ~ \chi_{1}^{\texttt{NL}} < h_{\nu} < \chi_{2}^{\texttt{NL}}  \\  0  ,  &  {\rm otherwise}  \end{cases}
\end{align}
where $ \chi_{1}^{\texttt{NL}}$ and $\chi_{2}^{\texttt{NL}}$ ($>  \chi_{1}^{\texttt{NL}}$) are the two roots of the equation $ \lambda^{\texttt{NL}} q^{\texttt{NL}} (x)  =  r(x) $, where $ q^{\texttt{NL}} (x) = \frac{ P_{s} T \left(  \frac{1}{1 + e^{-a (x P_{\rm avg} - b )}} - \Omega \right) }{ 1 - \Omega } $ and $ r (x) = \log_{2} \left(  1 +  \frac{ x P_{\rm avg} }{ \sigma^{2} } \right) $.
Also, the constant $\lambda^{\texttt{NL}} > 0$ is determined such that $ \mathbb{E} [   Q_{\nu}^{\texttt{NL}} ( P_{\rm avg} , \varrho_{\nu}^{\texttt{NL}} ) ]  = Q$.
Note that the existing mode switching result of (\ref{ms_NL}) can be considered as a special case of our result in Theorem \ref{thm_1} (or Theorem \ref{thm_2}) for the Case 3 (or Case 3').


\begin{figure}
    \centering
    \subfigure[Dynamic power splitting for the linear EH, eq. (\ref{rho_L}) \cite{Liu}]
    {
        \includegraphics[width=0.45\textwidth]{figure/insight_dps_L_csir.eps}
        \label{fig1_a}
    }
    \subfigure[Mode switching for the nonlinear EH, eq. (\ref{ms_NL}) \cite{Kang_2}]
    {
        \includegraphics[width=0.45\textwidth]{figure/insight_ms_NL_csir.eps}
        \label{fig1_b}
    }
    \subfigure[Dynamic power splitting for the nonlinear EH, eq. (\ref{rho_NL}) (proposed)]
    {
        \includegraphics[width=0.45\textwidth]{figure/insight_dps_NL_csir.eps}
        \label{fig1_c}
    }
    \caption{Comparison of the proposed and existing schemes for the case of CSIR.}
    \label{fig1}
\end{figure}

In Fig. \ref{fig1}, we illustrate the proposed and existing schemes.
In this figure, for notational simplicity, we focus on a particular fading state, and thus, we drop the index $\nu$ from the relevant expressions.
Also, the term ``PS" means the power splitting, i.e., both ID and EH.
In Fig. \ref{fig1_c}, $x_{1}^{\texttt{NL}}$, $( x_{2}^{\texttt{NL}} , x_{4}^{\texttt{NL}} )$, and $x_{3}^{\texttt{NL}}$ denote the roots of the equations 
$ \phi(x) = \frac{1}{4}$, $ \lambda_{\texttt{NL}} f(x) = g(0)$, and $ \lambda_{\texttt{NL}} f(0) = g(x)$, respectively.
For the illustration purpose, we assume that $ x_{j}^{\texttt{NL}} < x_{j+1}^{\texttt{NL}} $, $j = 1,2,3$.
%From the comparison in Fig. \ref{fig1} and the results of (\ref{rho_NL}), (\ref{rho_L}), and (\ref{ms_NL}), 
Comparing the proposed and existing schemes, we can obtain the following insights:
\begin{itemize}
\item From Figs. \ref{fig1_a} and \ref{fig1_c}, and the results of (\ref{rho_NL}) and (\ref{rho_L}), one can see that the optimal dynamic power splitting schemes for the linear EH and the nonlinear EH are different.
    For example, for the case of linear EH, the received power is used for the two different purposes: only for ID with $\rho^{\texttt{L}} = 0$ or for both ID and EH with $0 < \rho^{\texttt{L}} < 1$. Thus, in the linear EH, there are \textit{two} different regions for the optimal dynamic power splitting. On the other hand, for the case of nonlinear EH, the received power is used for the three different purposes: only for ID with $\rho^{\texttt{NL}} = 0$, only for EH with $\rho^{\texttt{NL}} = 1$, or for both ID and EH with $0 < \rho^{\texttt{NL}} < 1$. Consequently, in the nonlinear EH, there are up to \textit{five} different regions for the optimal dynamic power splitting.
    Also, for the case of linear EH, the optimal power splitting ratio increases as the channel gain increases, and thus, the power used for EH increases.
    On the other hand, for the case of nonlinear EH, the optimal power splitting ratio (and also, the power used for EH) increases, and then, decreases as the channel gain increases.
        
\item From Figs. \ref{fig1_b} and \ref{fig1_c}, and the results of (\ref{rho_NL}) and (\ref{ms_NL}), one can see that for the case of nonlinear EH, the optimal dynamic power splitting scheme is different from the optimal mode switching scheme. For example, in the mode switching, the optimal power splitting ratio $\varrho_{\nu}^{\texttt{NL}}$ takes two \textit{binary} values between 0 and 1, i.e., $\varrho_{\nu}^{\texttt{NL}} \in \{ 0,1\}$.
    Thus, the received power is used for the two different purposes: only for EH or only for ID. Consequently, in the mode switching, there are \textit{three} different regions for the optimal power splitting. On the other hand, in the dynamic power splitting, the optimal power splitting ratio $\rho_{\nu}^{\texttt{NL}}$ is \textit{continuous} between 0 and 1, i.e., $ \rho_{\nu}^{\texttt{NL}} \in [ 0, 1 ]$. Also, the received power is used for the three different purposes: only for ID, only for EH, or for both ID and EH. Consequently, in the dynamic power splitting, there are up to \textit{five} different regions for the optimal power splitting.
\end{itemize}







==> Tex/comparison_with_ms.tex <==
\subsection{Comparisons to Existing Schemes}
%\vspace{-0.5em}
\label{sec_P_EH_comp}

In this subsection, to obtain new and useful insights, we compare the proposed scheme to the existing schemes of \cite{Kang_2}, \cite{Liu_dps}.
For comparison, in the following, we first present the existing dynamic power splitting scheme for the linear EH \cite[Proposition 4.1]{Liu_dps}:
\begin{align}
\label{rho_L}
\rho_{\nu}^{\texttt{L}}  =  \begin{cases} \rho_{{\rm o}, \nu}^{\texttt{L}}  ,  &  {\rm if}  ~  h_{\nu}  >  x_{1}^{\texttt{L}}  \\ 0, & {\rm otherwise}  \end{cases}
\end{align}
where $ \rho_{{\rm o}, \nu}^{\texttt{L}} = 1 - \frac{1}{h_{\nu} P} \left( \frac{1}{ \zeta \lambda^{\texttt{L}} } - \sigma^{2} \right) $.
%\begin{align}
%\rho_{{\rm o}, \nu}^{\texttt{L}} = 1 - \frac{1}{h_{\nu} P} \left( \frac{1}{ \zeta \lambda^{\texttt{L}} } - \sigma^{2} \right).
%\end{align}
Also, $x_{1}^{\texttt{L}} = \frac{1}{ P }  \left( \frac{1}{ \zeta \lambda^{\texttt{L}} } - \sigma^{2} \right)$.
The constant $ 0 < \lambda^{\texttt{L}} \leq \frac{1}{\zeta \sigma^{2}} $ is determined such that $\mathbb{E} [   Q_{\nu}^{\texttt{L}} ( P , \rho_{\nu}^{\texttt{L}} ) ]  = Q$.
Next, we present the existing mode switching scheme for the nonlinear EH \cite[Lemma 2]{Kang_2}:
\begin{align}
\label{ms_NL}
\varrho_{\nu}^{\texttt{NL}}  = \begin{cases}  1 ,  & {\rm if} ~ \chi_{1}^{\texttt{NL}} < h_{\nu} < \chi_{2}^{\texttt{NL}}  \\  0  ,  &  {\rm otherwise}  \end{cases}
\end{align}
where $ \chi_{1}^{\texttt{NL}}$ and $\chi_{2}^{\texttt{NL}}$ ($>  \chi_{1}^{\texttt{NL}}$) are the two roots of the equation $ \lambda^{\texttt{NL}} q^{\texttt{NL}} (x)  =  r(x) $, where $ q^{\texttt{NL}} (x) = \frac{ P_{s} T \left(  \frac{1}{1 + e^{-a (x P - b )}} - \Omega \right) }{ 1 - \Omega } $ and $ r (x) = \log_{2} \left(  1 +  \frac{ x P }{ \sigma^{2} } \right) $.
Also, the constant $\lambda^{\texttt{NL}} > 0$ is determined such that $ \mathbb{E} [   Q_{\nu}^{\texttt{NL}} ( P , \varrho_{\nu}^{\texttt{NL}} ) ]  = Q$.
Note that the existing mode switching result of (\ref{ms_NL}) can be considered as a special case of our result in Theorem \ref{thm_1} (or Theorem \ref{thm_2}) for the Case 3 (or Case 3$'$).


\begin{figure}
    \centering
    \subfigure[Dynamic power splitting for the linear EH, eq. (\ref{rho_L}) \cite{Liu_dps}]
    {
        \includegraphics[width=0.45\textwidth]{figure/insight_dps_L_csir.eps}
        \label{fig1_a}
    }
    \subfigure[Mode switching for the nonlinear EH, eq. (\ref{ms_NL}) \cite{Kang_2}]
    {
        \includegraphics[width=0.45\textwidth]{figure/insight_ms_NL_csir.eps}
        \label{fig1_b}
    }
    \subfigure[Dynamic power splitting for the nonlinear EH, eq. (\ref{rho_NL}) (proposed)]
    {
        \includegraphics[width=0.45\textwidth]{figure/insight_dps_NL_csir.eps}
        \label{fig1_c}
    }
    \caption{Comparison of the proposed and existing schemes for the case of CSIR.}
    \label{fig1}
\end{figure}

In Fig. \ref{fig1}, we illustrate the proposed and existing schemes.
In this figure, for notational simplicity, we focus on a particular fading state, and thus, we drop the index $\nu$ from the relevant expressions.
Also, in Fig. \ref{fig1}, the term ``PS'' means the power splitting, i.e., both ID and EH.
In Fig. \ref{fig1_c}, $x_{1}^{\texttt{NL}}$, $( x_{2}^{\texttt{NL}} , x_{4}^{\texttt{NL}} )$, and $x_{3}^{\texttt{NL}}$ denote the roots of the equations
$ \gamma(x) = \frac{1}{4}$, $ \lambda_{\texttt{NL}} f(x) = g(0)$, and $ \lambda_{\texttt{NL}} f(0) = g(x)$, respectively.
For the illustration purpose, we assume that $ x_{j}^{\texttt{NL}} < x_{j+1}^{\texttt{NL}} $, $j = 1,2,3$.
%From the comparison in Fig. \ref{fig1} and the results of (\ref{rho_NL}), (\ref{rho_L}), and (\ref{ms_NL}),

To obtain the direct and useful insights that are related to the distance,
we consider a practical distance-based channel model of \cite{Huang15}:
$h = 1 - \exp\left( - \frac{a_{t} a_{r}}{ (c/f_{c})^{2} d^{2} } \right)$,
where $a_{t}$ is the aperture of the transmit antenna; $a_{r}$ is the aperture of the receive antenna; $c$ is the speed of light; $f_{c}$ is the carrier frequency; and $d$ is the distance between the transmitter and the receiver.
Then, comparing the proposed and existing schemes, we can obtain the following insights:
\begin{itemize}
\item From Figs. \ref{fig1_a} and \ref{fig1_c}, and the results of (\ref{rho_NL}) and (\ref{rho_L}), one can see that the optimal dynamic power splitting schemes for the linear EH and the nonlinear EH are fundamentally different.
    For example, for the case of linear EH, the received power is used for the two different purposes: only for ID with $\rho^{\texttt{L}} = 0$ or for both ID and EH with $0 < \rho^{\texttt{L}} < 1$. Thus, in the linear EH, there are \textit{two} different regions for the optimal dynamic power splitting. On the other hand, for the case of nonlinear EH, the received power is used for the three different purposes: only for ID with $\rho^{\texttt{NL}} = 0$, only for EH with $\rho^{\texttt{NL}} = 1$, or for both ID and EH with $0 < \rho^{\texttt{NL}} < 1$. Consequently, in the nonlinear EH, there are up to \textit{five} different regions for the optimal dynamic power splitting.
    Also, for the case of linear EH, the optimal power splitting ratio $\rho^{\texttt{NL}}$ increases as the distance $d$ decreases (or the channel gain $h$ increases), and thus, the power used for EH increases.
    On the other hand, for the case of nonlinear EH, the optimal power splitting ratio $\rho^{\texttt{NL}}$ (and thus, the power used for EH) increases, and then, decreases as the distance $d$ decreases.

\item From Figs. \ref{fig1_b} and \ref{fig1_c}, and the results of (\ref{rho_NL}) and (\ref{ms_NL}), one can see that for the case of nonlinear EH, the optimal dynamic power splitting scheme is very different from the optimal mode switching scheme. For example, in the mode switching, the optimal power splitting ratio $\varrho^{\texttt{NL}}$ takes two \textit{binary} values between 0 and 1, i.e., $\varrho^{\texttt{NL}} \in \{ 0,1\}$.
    Thus, the received power is used for the two different purposes: only for EH or only for ID. Consequently, in the mode switching, there are \textit{three} different regions for the optimal power splitting. On the other hand, in the dynamic power splitting, the optimal power splitting ratio $\rho^{\texttt{NL}}$ is \textit{continuous} between 0 and 1, i.e., $ \rho^{\texttt{NL}} \in [ 0, 1 ]$. Also, the received power is used for the three different purposes: only for ID, only for EH, or for both ID and EH. Consequently, in the dynamic power splitting, there are up to \textit{five} different regions for the optimal power splitting.
\end{itemize}

==> Tex/numerical_result_old.tex <==
\vspace{-1.5em}
\section{Numerical Results}
\vspace{-0.5em}
\label{numerical_result}

In this section, the performance of the proposed scheme is demonstrated through the numerical results and it is compared to that of the existing schemes of \cite{Liu}, \cite{Kang_2}, \cite{Kang_3}.
The R-E tradeoff performance is evaluated based on the nonlinear EH model of (\ref{Q_NL}).
In the simulations, we set $a = 6400$ and $b = 0.003$ as in \cite{Boshkovska15}, \cite{Boshkovska17_2}, which were obtained based on the measurement data of \cite{Mayaram08}.
Also, we set $ P_{s} = \mathbb{E} [ h_{\nu} ] P_{\rm avg} $.
The block duration is normalized to unity, i.e., $T = 1$ second.
Also, the long-term and short-term power thresholds are set to $P_{\rm avg} = 2 $ W and $P_{\max} = 2 P_{\rm avg} = 4$ W, respectively.
Unless stated otherwise, the fading blocks are generated randomly according to the Rician channel model as follows: $\eta_{\nu} = \sqrt{\frac{\alpha}{\alpha+1}} \bar{\eta}  + \sqrt{\frac{1}{\alpha+1}} \tilde{\eta}_{\nu} $, $\forall \nu$, where $\eta_{\nu}$ is the channel at the fading state $\nu$. Thus, the channel power gain $h_{\nu}$ at that state can be obtained as $h_{\nu} = | \eta_{\nu} |^{2}$.
Also, $\alpha$ is the Rician factor, and $\bar{\eta}$ and $\tilde{\eta}_{\nu} \sim \mathcal{CN} (0, \sigma_{h}^{2})$ are the line-of-sight and scattering components, respectively.
We set $\alpha = 1$ and $| \bar{\eta} |^{2} = \sigma_{h}^{2} = - 28$ dBW.




In Figs. \ref{fig2} and \ref{fig3}, the R-E regions of the proposed and existing schemes are shown for the cases of no CSIT and CSIT, respectively, when $ \frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} \in \{ 0, 10, 20 \} $ dB. From Figs. \ref{fig2} and \ref{fig3}, one can see that the proposed schemes significantly outperform the existing schemes in terms of the R-E tradeoff performance.
For the case of CSIT, only with the long-term power constraint, the proposed optimal scheme yields the best performance.
As expected from Lemma \ref{lem_optimality}, the proposed suboptimal scheme provides the optimal performance in the low SNR range (e.g., when $ \frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 0 $ dB).
Even in the moderate and high SNR ranges (e.g., when $ \frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = \{ 10, 20 \} $ dB),
this scheme performs very well and its performance is almost the same as the optimal performance.
%The performance of this scheme is essentially the same as the optimal performance
%The existing mode switching scheme for the nonlinear EH is suboptimal because the received power is used only for ID or only for EH.
There exists a tradeoff between the existing schemes.
In the higher rate regime, the existing dynamic power splitting scheme for the linear EH performs better than the existing mode switching scheme for the nonlinear EH.
On the other hand, in the lower rate regime, the existing dynamic power splitting scheme for the linear EH is even worse than the existing mode switching scheme for the nonlinear EH
due to the inaccurate or mismatched rules for power splitting and/or power allocation.

%Fig. shows the R-E regions of the proposed and existing schemes for the case of CSIT when $ \frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} \in \{ 0, 10, 20 \} $ dB.
%It can be seen that the R-E regions of the proposed schemes substantially larger than those of the existing schemes.
%Only with the long-term power constraint, the proposed scheme has the largest R-E region.
%As expected from Lemma \ref{lem_optimality_2}, the proposed suboptimal scheme has the same R-E region as the optimal scheme in the low SNR region.
%The R-E region of this scheme is almost the same as that of the optimal scheme even in the moderate and high SNR regimes.
%In the high (or low) rate regime, the existing dynamic power splitting scheme for the linear EH is better (or worse) than the existing mode switching scheme for the nonlinear EH.

\begin{figure*}
    \centering
    \subfigure[When $\frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 0$ dB]
    {
        \includegraphics[width=0.31\textwidth]{figure/R_E_tradeoff_csir_0db.eps}
        \label{fig2_a}
    }
    \subfigure[When $\frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 10$ dB]
    {
        \includegraphics[width=0.31\textwidth]{figure/R_E_tradeoff_csir_10db.eps}
        \label{fig2_b}
    }
    \subfigure[When $\frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 20$ dB]
    {
        \includegraphics[width=0.31\textwidth]{figure/R_E_tradeoff_csir_20db.eps}
        \label{fig2_c}
    }
    \caption{R-E regions of the proposed and existing schemes for the case of no CSIT.}
    \label{fig2}
\end{figure*}

\begin{figure*}
    \centering
    \subfigure[When $\frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 0$ dB]
    {
        \includegraphics[width=0.31\textwidth]{figure/R_E_tradeoff_csit_0db.eps}
        \label{fig3_a}
    }
    \subfigure[When $\frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 10$ dB]
    {
        \includegraphics[width=0.31\textwidth]{figure/R_E_tradeoff_csit_10db.eps}
        \label{fig3_b}
    }
    \subfigure[When $\frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 20$ dB]
    {
        \includegraphics[width=0.31\textwidth]{figure/R_E_tradeoff_csit_20db.eps}
        \label{fig3_c}
    }
    \caption{R-E regions of the proposed and existing schemes for the case of CSIT.}
    \label{fig3}
\end{figure*}


Considering the practical applications such as the Internet-of-Things (IoT) with implanted bio and/or wearable sensors, in Fig. \ref{fig4}, we investigate the impact of the receiver mobility on the R-E tradeoff performance. In Fig. \ref{fig4}, the R-E regions of the proposed and existing schemes are shown for the cases of no CSIT and CSIT when $ \frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 15 $ dB.
In this figure, we model the channel power gain as follows: $h_{\nu} = 1 - e^{ - \frac{a_{t} a_{r}}{ (c/f_{c})^{2} d_{\nu}^{2} } }$, $\forall \nu$ \cite{Huang15},
where $a_{t}$ is the aperture of the transmit antenna; $a_{r}$ the aperture of the receive antenna; $c$ the speed of light; and $d_{\nu}$ the distance between the transmitter and the receiver.
Assuming that the receiver is a small sensor, we set $a_{t} = 0.5$ m, $a_{r} = 0.01$ m, and $f_{c} = 2.4$ GHz \cite{Kim16}--\cite{Kang}.
Also, considering the mobility of the receiver, we set the distance $d_{\nu}$ in the current fading state $\nu$ as follows: $d_{\nu} = d_{\nu'} + \beta_{\nu} v_{\max} T$,
where $d_{\nu'}$ is the distance in the previous fading state $\nu'$; $v_{\max}$ the maximum speed; and $\beta_{\nu}$ the parameter accounting for the directionality.
We set the initial distance to $15$ m and we select $\beta_{\nu}$ randomly over the range $[-1,1]$. Also, we set $v_{\max} = 0.1$ m/s.
From Fig. \ref{fig4}, it can be seen that in the scenario of the receiver mobility, the proposed schemes is much better than the existing schemes,
which clearly shows the significant advantages of the proposed schemes over the existing schemes in the practical applications.
%since the fading channel fluctuates more rapidly.
%Only with the long-term power constraint, the proposed optimal scheme substantially enhance the performance.
%Also, the proposed suboptimal scheme yields almost the same performance as the optimal scheme.
%Directly using the existing schemes results in the severely degraded performance,
%which reveals the limitations of the existing schemes in the practical application scenario.


\begin{figure*}
    \centering
    \subfigure[For the case of no CSIT]
    {
        \includegraphics[width=0.35\textwidth]{figure/RE_tradeoff_csir_15db.eps}
        \label{fig4_a}
    }
    \subfigure[For the case of CSIT]
    {
        \includegraphics[width=0.35\textwidth]{figure/RE_tradeoff_csit_15db.eps}
        \label{fig4_b}
    }
    \caption{R-E regions of the proposed and existing schemes with the receiver mobility when $ \frac{ \mathbb{E} [ h_{\nu} ] P_{\rm avg} } {\sigma^{2}} = 15 $ dB.}
    \label{fig4}
\end{figure*}


























